Graph Queries from Natural Language using Constrained Language Models and Visual Editing

Querying knowledge bases using ontologies is usually performed using dedicated query languages, question-answering systems, or visual query editors for Knowledge Graphs. We propose a novel approach that enables users to query the knowledge graph by specifying prototype graphs in natural language and visually editing them. This approach enables non-experts to formulate queries without prior knowledge of the ontology and specific query languages. Our approach converts natural language to these prototype graphs by utilizing a two-step constrained language model generation based on semantically similar features within an ontology. The resulting prototype graph serves as the building block for further user refinements within a dedicated visual query builder. Our approach consistently generates a valid SPARQL query within the constraints imposed by the ontology, without requiring any additional corrections to the syntax or classes and links used. Unlike related language models approaches, which often require multiple iterations to fix invalid syntax, non-existent classes, and non-existent links, our approach achieves this consistently. We evaluate the performance of our system using graph retrieval on synthetic queries, comparing multiple metrics, models, and ontologies. We further validate our system through a preliminary user study. By utilizing our constrained pipeline, we show that the system can perform efficient and accurate retrieval using more efficient models compared to other approaches.

==> figures/erl_constrained.tex <==
\usetikzlibrary {arrows.meta, graphs, shapes.misc, matrix, quotes, patterns, shapes.arrows, shapes.misc, positioning, calc, fit, bending}

\begin{tikzpicture}[
    scale=\erlsize, transform shape,
    entity/.style={rectangle, draw=black!90,  fill=black!20, minimum size=1cm,  text width=2.6cm, font={\LARGE}, align=center},
    every edge/.append style ={
        inner sep=0pt, auto,
        align=left},
    every new --/.style={line width=0.5pt},
  ]
  \node (p1) [entity] {person};
  \node (bel_p1) [below=of p1]{};
  \node (p2) [entity, right=1.75cm of bel_p1, text width=2cm, draw=red] {person};
  \node (uni) [entity, right=4cm of p1, draw=red] {university};
  \graph [use existing nodes] {
  p1.east--[out=0,in=180, draw=red]p2.west;
  p1.east--[out=0,in=180, ]uni.west;
  p2.east--[out=0,in=180]uni.west;
  };
\end{tikzpicture}

==> figures/erl_edit.tex <==
\usetikzlibrary{patterns,shapes.arrows}
\usetikzlibrary {arrows.meta, graphs, shapes.misc, matrix, quotes, patterns, shapes.arrows, shapes.misc, positioning, calc, fit, bending}

\begin{tikzpicture}[
    scale=\erlsize, transform shape,
    entity/.style={rectangle, draw=black!90,  fill=black!20, minimum size=1cm,  text width=2cm, font={\LARGE}, align=center},
    every edge/.append style ={
        inner sep=0pt, auto,
        align=left},
    every new --/.style={line width=0.5pt},
  ]
  \node (p1) [entity] {person};
  \node (bel_p1) [below=of p1]{};
  \node (p2) [entity, right=1.6cm of bel_p1] {person};
  \node (uni) [entity, right=3.5cm of p1,  text width=3cm] {university};
  \node (country) [entity, right=4.5cm of p2, draw=OliveDrab, fill=OliveDrab!10] {country};
  \graph [use existing nodes] {
  p1.east--[out=0,in=180]p2.west;
  p1.east--[out=0,in=180, ]uni.west;
  p2.east--[out=0,in=180]uni.west;
  uni.east--[out=0,in=180, draw=OliveDrab]country.west;
  p2.east--[out=0,in=180, draw=OliveDrab]country.west;
  };

\end{tikzpicture}

==> figures/erl_ex.tex <==
\usetikzlibrary{patterns,shapes.arrows}
\usetikzlibrary {arrows.meta, graphs, shapes.misc, matrix, quotes, patterns, shapes.arrows, shapes.misc, positioning, calc, fit, bending}

\begin{tikzpicture}[
    scale=\erlsize, transform shape,
    entity/.style={rectangle, draw=black!90,  fill=black!20, minimum size=1cm,  text width=1.7cm, font={\LARGE}, align=center},
    every edge/.append style ={
        inner sep=0pt, auto,
        align=left},
    every new --/.style={line width=0.5pt},
  ]
  \node (p1) [entity] {\erlperson};
  \node (bel_p1) [below=of p1]{};
  \node (p2) [entity, right=1.6cm of bel_p1] {\erlchild};
  \node (uni) [entity, right=4cm of p1] {\erluni};
  \node (country) [entity, right=4cm of p2] {\erlcountry};
  \graph [use existing nodes] {
  p1.east--[out=0,in=180]p2.west;
  p1.east--[out=0,in=180, ]uni.west;
  p2.east--[out=0,in=180]uni.west;
  uni.east--[out=0,in=180]country.west;
  p2.east--[out=0,in=180]country.west;
  };

\end{tikzpicture}

==> figures/erl_unconstrained.tex <==
\usetikzlibrary {arrows.meta, graphs, shapes.misc, matrix, quotes, patterns, shapes.arrows, shapes.misc, positioning, calc, fit, bending}

\begin{tikzpicture}[
    scale=\erlsize, transform shape,
    entity/.style={rectangle, draw=black!90,  fill=black!20, minimum size=1cm,  text width=3cm, font={\LARGE}, align=center},
    every edge/.append style ={
        inner sep=0pt, auto,
        align=left},
    every new --/.style={line width=0.5pt},
  ]
  \node (p1) [entity] {person};
  \node (bel_p1) [below=of p1]{};
  \node (p2) [entity, below=of p1] {child};
  \node (uni) [entity, right=2cm of p1] {college};
  \graph [use existing nodes] {
  p1.west--[out=180,in=180, ]p2.west;
  p1.east--[out=0,in=180, ]uni.west;
  p2.east--[out=0,in=180]uni.west;
  };

\end{tikzpicture}

==> generated/tables/compare_gen_query.tex <==
\begin{table}
\caption{Comparison of query generation methods for LLama 3.2 3B on DBpedia with one shot prompts.}
\label{tab:compare_gen_query}
\begin{tabular}{lllrr}
\toprule
 &  &  & Mean $F_{1,node}$ & Mean $GED_{s}$ \\
$k$ & Query Origin & Stage &  &  \\
\midrule
\multirow[t]{6}{*}{3} & \multirow[t]{2}{*}{human} & aligned & 0.63 & 0.53 \\
 &  & raw & 0.71 & 0.53 \\
\cline{2-5}
 & \multirow[t]{2}{*}{llama} & aligned & 0.71 & 0.49 \\
 &  & raw & 0.71 & 0.34 \\
\cline{2-5}
 & \multirow[t]{2}{*}{templated} & aligned & 0.81 & 0.55 \\
 &  & raw & 0.81 & 0.53 \\
\cline{1-5} \cline{2-5}
\multirow[t]{6}{*}{5} & \multirow[t]{2}{*}{human} & aligned & 0.75 & 0.52 \\
 &  & raw & 0.77 & 0.24 \\
\cline{2-5}
 & \multirow[t]{2}{*}{llama} & aligned & 0.71 & 0.41 \\
 &  & raw & 0.73 & 0.26 \\
\cline{2-5}
 & \multirow[t]{2}{*}{templated} & aligned & 0.79 & 0.48 \\
 &  & raw & 0.78 & 0.46 \\
\cline{1-5} \cline{2-5}
\bottomrule
\end{tabular}
\end{table}


==> generated/tables/compare_model_BTO.tex <==
\begin{table}
\caption{Comparison of models for BTO}
\label{tab:compare_model_BTO}
\begin{tabular}{lllllrrr}
\toprule
 &  &  &  &  & $F_{1,node}$ & $GED_{s}$ & $F_{1,rel.}$  \\
$k$ & Stage & Prompt Type & Version \& Size & Percentile &  &  &  \\
\midrule
\multirow[t]{30}{*}{2} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.00 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.33 & 1.00 \\
 &  &  &  & 0.750000 & 0.50 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.00 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.33 & 1.00 \\
 &  &  &  & 0.750000 & 0.67 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.33 & 1.00 \\
 &  &  &  & 0.750000 & 0.50 & 0.33 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.33 & 1.00 \\
 &  &  &  & 0.750000 & 0.50 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.33 & 1.00 \\
 &  &  &  & 0.750000 & 0.50 & 0.33 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 0.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.50 & 0.33 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.00 & 0.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.00 & 0.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.00 & 0.00 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{30}{*}{3} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.40 & 0.40 & 0.67 \\
 &  &  &  & 0.500000 & 0.67 & 0.60 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.50 & 0.33 & 0.67 \\
 &  &  &  & 0.500000 & 0.67 & 0.63 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.40 & 0.40 & 0.50 \\
 &  &  &  & 0.500000 & 0.67 & 0.60 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.40 & 0.40 & 1.00 \\
 &  &  &  & 0.500000 & 0.67 & 0.60 & 1.00 \\
 &  &  &  & 0.750000 & 0.80 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.22 & 0.67 \\
 &  &  &  & 0.500000 & 0.33 & 0.40 & 1.00 \\
 &  &  &  & 0.750000 & 0.73 & 0.60 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.40 & 0.57 & 0.50 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.38 & 0.50 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.14 & 0.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.21 & 0.75 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.21 & 0.50 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{30}{*}{5} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.50 & 0.17 & 0.40 \\
 &  &  &  & 0.500000 & 0.60 & 0.33 & 0.67 \\
 &  &  &  & 0.750000 & 0.80 & 0.83 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.44 & 0.33 & 0.67 \\
 &  &  &  & 0.500000 & 0.67 & 0.44 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.86 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.59 & 0.33 & 0.86 \\
 &  &  &  & 0.500000 & 0.75 & 0.51 & 0.86 \\
 &  &  &  & 0.750000 & 0.82 & 0.72 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.52 & 0.31 & 0.75 \\
 &  &  &  & 0.500000 & 0.67 & 0.53 & 0.86 \\
 &  &  &  & 0.750000 & 0.77 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.25 & 0.22 & 0.75 \\
 &  &  &  & 0.500000 & 0.40 & 0.40 & 0.86 \\
 &  &  &  & 0.750000 & 0.57 & 0.56 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.43 & 0.58 & 0.75 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.50 & 0.44 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.38 & 0.89 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & -0.10 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.44 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & -0.10 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.44 & 1.00 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{30}{*}{7} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.67 & 0.56 & 0.63 \\
 &  &  &  & 0.500000 & 0.72 & 0.58 & 0.66 \\
 &  &  &  & 0.750000 & 0.78 & 0.60 & 0.70 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.33 & 0.25 & 0.67 \\
 &  &  &  & 0.500000 & 0.67 & 0.33 & 0.80 \\
 &  &  &  & 0.750000 & 0.86 & 0.57 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.50 & 0.16 & 0.58 \\
 &  &  &  & 0.500000 & 0.64 & 0.31 & 0.72 \\
 &  &  &  & 0.750000 & 0.78 & 0.47 & 0.86 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.62 & 0.77 & 1.00 \\
 &  &  &  & 0.500000 & 0.62 & 0.77 & 1.00 \\
 &  &  &  & 0.750000 & 0.62 & 0.77 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.29 & 0.48 & 0.85 \\
 &  &  &  & 0.500000 & 0.39 & 0.58 & 0.90 \\
 &  &  &  & 0.750000 & 0.48 & 0.67 & 0.95 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.21 & 0.19 & 0.17 \\
 &  &  &  & 0.500000 & 0.43 & 0.38 & 0.33 \\
 &  &  &  & 0.750000 & 0.64 & 0.58 & 0.50 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.00 & 0.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.10 & 0.23 \\
 &  &  &  & 0.500000 & 0.00 & 0.20 & 0.46 \\
 &  &  &  & 0.750000 & 0.00 & 0.30 & 0.69 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.46 & 1.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.46 & 1.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.46 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.12 & 0.25 \\
 &  &  &  & 0.500000 & 0.00 & 0.23 & 0.50 \\
 &  &  &  & 0.750000 & 0.00 & 0.35 & 0.75 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{2} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.28 & 0.43 & 0.80 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.41 & 0.49 & 0.83 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.18 & 0.35 & 0.78 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.33 & 0.46 & 0.82 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.19 & 0.39 & 0.82 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.35 & 0.27 & 0.18 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.21 & 0.23 & 0.33 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.01 & 0.06 & 0.16 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.01 & 0.07 & 0.19 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.05 & 0.10 & 0.21 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{3} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.65 & 0.59 & 0.73 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.65 & 0.61 & 0.77 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.66 & 0.59 & 0.73 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.59 & 0.63 & 0.91 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.37 & 0.46 & 0.83 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.24 & 0.20 & 0.24 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.22 & 0.22 & 0.25 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.05 & 0.07 & 0.20 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.00 & 0.09 & 0.27 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.07 & 0.14 & 0.27 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{5} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.60 & 0.46 & 0.68 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.63 & 0.55 & 0.80 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.72 & 0.55 & 0.84 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.63 & 0.49 & 0.81 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.41 & 0.43 & 0.83 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.23 & 0.23 & 0.32 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.26 & 0.27 & 0.31 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.07 & 0.18 & 0.38 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.00 & 0.11 & 0.35 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.01 & 0.12 & 0.34 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{7} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.72 & 0.58 & 0.66 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.57 & 0.40 & 0.73 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.64 & 0.31 & 0.72 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.62 & 0.77 & 1.00 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.39 & 0.58 & 0.90 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.43 & 0.38 & 0.33 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.09 & 0.02 & 0.04 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.00 & 0.20 & 0.46 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.00 & 0.46 & 1.00 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.00 & 0.23 & 0.50 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\bottomrule
\end{tabular}
\end{table}


==> generated/tables/compare_model_DBpedia.tex <==
\begin{table}
\caption{Comparison of models for DBpedia}
\label{tab:compare_model_DBpedia}
\begin{tabular}{lllllrrr}
\toprule
 &  &  &  &  & $F_{1,node}$ & $GED_{s}$ & $F_{1,rel.}$  \\
$k$ & Stage & Prompt Type & Version \& Size & Percentile &  &  &  \\
\midrule
\multirow[t]{30}{*}{2} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.50 & 0.25 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.40 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.14 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.33 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.40 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.33 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.45 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.50 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.40 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.40 & 0.67 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 0.67 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.20 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 0.00 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{30}{*}{3} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.67 & 0.29 & 0.50 \\
 &  &  &  & 0.500000 & 0.80 & 0.50 & 0.80 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.67 & 0.22 & 0.50 \\
 &  &  &  & 0.500000 & 0.80 & 0.56 & 0.80 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.40 & 0.20 & 0.50 \\
 &  &  &  & 0.500000 & 0.80 & 0.50 & 0.67 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.40 & 0.33 & 0.50 \\
 &  &  &  & 0.500000 & 0.67 & 0.57 & 0.80 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.40 & 0.29 & 0.50 \\
 &  &  &  & 0.500000 & 0.67 & 0.50 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.67 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.40 & 0.33 \\
 &  &  &  & 0.750000 & 1.00 & 0.60 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.67 & 0.29 & 0.21 \\
 &  &  &  & 0.500000 & 0.93 & 0.57 & 0.67 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.50 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.40 & 0.40 \\
 &  &  &  & 0.750000 & 1.00 & 0.60 & 0.80 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.40 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.67 & 0.40 & 0.50 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.33 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.67 & 0.29 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.60 & 0.40 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{30}{*}{5} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.67 & 0.25 & 0.60 \\
 &  &  &  & 0.500000 & 0.80 & 0.44 & 0.80 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.67 & 0.22 & 0.60 \\
 &  &  &  & 0.500000 & 0.89 & 0.45 & 0.80 \\
 &  &  &  & 0.750000 & 1.00 & 0.70 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.60 & 0.26 & 0.57 \\
 &  &  &  & 0.500000 & 0.80 & 0.44 & 0.75 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.50 & 0.25 & 0.57 \\
 &  &  &  & 0.500000 & 0.80 & 0.45 & 0.75 \\
 &  &  &  & 0.750000 & 1.00 & 0.70 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.44 & 0.22 & 0.67 \\
 &  &  &  & 0.500000 & 0.75 & 0.45 & 0.75 \\
 &  &  &  & 0.750000 & 1.00 & 0.78 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.60 & 0.13 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.30 & 0.29 \\
 &  &  &  & 0.750000 & 1.00 & 0.55 & 0.80 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.67 & 0.22 & 0.25 \\
 &  &  &  & 0.500000 & 0.89 & 0.45 & 0.67 \\
 &  &  &  & 0.750000 & 1.00 & 0.70 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.59 & 0.11 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.33 & 0.25 \\
 &  &  &  & 0.750000 & 1.00 & 0.56 & 0.75 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.44 & 0.11 & 0.00 \\
 &  &  &  & 0.500000 & 0.75 & 0.33 & 0.25 \\
 &  &  &  & 0.750000 & 1.00 & 0.60 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.29 & 0.10 & 0.00 \\
 &  &  &  & 0.500000 & 0.67 & 0.27 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.56 & 0.75 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{30}{*}{7} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.55 & 0.17 & 0.55 \\
 &  &  &  & 0.500000 & 0.73 & 0.31 & 0.80 \\
 &  &  &  & 0.750000 & 0.91 & 0.54 & 0.92 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.61 & 0.20 & 0.60 \\
 &  &  &  & 0.500000 & 0.86 & 0.43 & 0.83 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.60 & 0.21 & 0.55 \\
 &  &  &  & 0.500000 & 0.83 & 0.38 & 0.80 \\
 &  &  &  & 0.750000 & 0.92 & 0.60 & 0.91 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.55 & 0.24 & 0.62 \\
 &  &  &  & 0.500000 & 0.83 & 0.38 & 0.83 \\
 &  &  &  & 0.750000 & 1.00 & 0.64 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.44 & 0.25 & 0.60 \\
 &  &  &  & 0.500000 & 0.75 & 0.44 & 0.83 \\
 &  &  &  & 0.750000 & 1.00 & 0.69 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.60 & 0.08 & 0.15 \\
 &  &  &  & 0.500000 & 0.77 & 0.27 & 0.33 \\
 &  &  &  & 0.750000 & 0.86 & 0.46 & 0.83 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.71 & 0.22 & 0.20 \\
 &  &  &  & 0.500000 & 0.86 & 0.38 & 0.62 \\
 &  &  &  & 0.750000 & 1.00 & 0.62 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.67 & 0.14 & 0.00 \\
 &  &  &  & 0.500000 & 0.83 & 0.31 & 0.33 \\
 &  &  &  & 0.750000 & 0.92 & 0.50 & 0.83 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.55 & 0.13 & 0.00 \\
 &  &  &  & 0.500000 & 0.83 & 0.31 & 0.40 \\
 &  &  &  & 0.750000 & 1.00 & 0.62 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.36 & 0.08 & 0.00 \\
 &  &  &  & 0.500000 & 0.62 & 0.27 & 0.00 \\
 &  &  &  & 0.750000 & 0.93 & 0.54 & 0.92 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{2} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.67 & 0.57 & 0.62 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.64 & 0.53 & 0.67 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.48 & 0.47 & 0.62 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.49 & 0.50 & 0.66 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.51 & 0.51 & 0.64 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.68 & 0.51 & 0.41 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.65 & 0.49 & 0.47 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.49 & 0.38 & 0.32 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.44 & 0.39 & 0.39 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.45 & 0.31 & 0.14 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{3} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.75 & 0.52 & 0.68 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.75 & 0.53 & 0.69 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.71 & 0.51 & 0.65 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.66 & 0.54 & 0.71 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.64 & 0.53 & 0.71 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.75 & 0.43 & 0.40 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.77 & 0.55 & 0.60 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.71 & 0.42 & 0.38 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.63 & 0.43 & 0.44 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.58 & 0.34 & 0.21 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{5} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.75 & 0.45 & 0.74 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.80 & 0.48 & 0.75 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.73 & 0.46 & 0.73 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.70 & 0.48 & 0.77 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.66 & 0.49 & 0.76 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.76 & 0.35 & 0.42 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.80 & 0.48 & 0.60 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.71 & 0.35 & 0.40 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.69 & 0.38 & 0.47 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.61 & 0.32 & 0.30 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{7} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.71 & 0.36 & 0.71 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.78 & 0.42 & 0.74 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.74 & 0.41 & 0.71 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.75 & 0.44 & 0.77 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.67 & 0.46 & 0.76 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.72 & 0.30 & 0.46 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.80 & 0.42 & 0.60 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.76 & 0.33 & 0.43 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.72 & 0.40 & 0.53 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.61 & 0.32 & 0.34 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\bottomrule
\end{tabular}
\end{table}


==> generated/tables/compare_model_DNB.tex <==
\begin{table}
\caption{Comparison of models for DNB}
\label{tab:compare_model_DNB}
\begin{tabular}{llllrr}
\toprule
 &  &  &  & $F_1$ & $GED_{s}$ \\
$k$ & Stage & Prompt Type & Version \& Size &  &  \\
\midrule
\multirow[t]{3}{*}{3.000000} & aligned & one shot &  3B  & 0.20 & 0.22 \\
\cline{2-6} \cline{3-6}
 & constrained & one shot &  3B  & 0.00 & -0.01 \\
\cline{2-6} \cline{3-6}
 & raw & one shot &  3B  & 0.10 & 0.03 \\
\cline{1-6} \cline{2-6} \cline{3-6}
\bottomrule
\end{tabular}
\end{table}


==> generated/tables/compare_model_UniProt.tex <==
\begin{table}
\caption{Comparison of models for UniProt}
\label{tab:compare_model_UniProt}
\begin{tabular}{lllllrrr}
\toprule
 &  &  &  &  & $F_{1,node}$ & $GED_{s}$ & $F_{1,rel.}$  \\
$k$ & Stage & Prompt Type & Version \& Size & Percentile &  &  &  \\
\midrule
\multirow[t]{30}{*}{2} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.50 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.40 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 0.67 & 0.67 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.50 & 0.33 & 0.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.33 & 0.67 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.22 & 0.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.33 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.33 & 0.67 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{30}{*}{3} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.40 & 0.40 & 1.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.60 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.83 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.33 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.67 & 0.57 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.33 & 0.29 & 0.67 \\
 &  &  &  & 0.500000 & 0.67 & 0.40 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.29 & 0.83 \\
 &  &  &  & 0.500000 & 0.40 & 0.43 & 1.00 \\
 &  &  &  & 0.750000 & 0.80 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.27 & 0.20 & 0.67 \\
 &  &  &  & 0.500000 & 0.50 & 0.40 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.55 & 0.40 & 0.50 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.40 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.20 & 0.50 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.40 \\
 &  &  &  & 0.750000 & 0.00 & 0.40 & 0.73 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.750000 & 0.00 & 0.20 & 0.50 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{30}{*}{5} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.50 & 0.33 & 0.67 \\
 &  &  &  & 0.500000 & 0.67 & 0.44 & 0.86 \\
 &  &  &  & 0.750000 & 0.80 & 0.78 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.43 & 0.33 & 0.75 \\
 &  &  &  & 0.500000 & 0.60 & 0.48 & 0.86 \\
 &  &  &  & 0.750000 & 1.00 & 0.78 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.38 & 0.32 & 0.73 \\
 &  &  &  & 0.500000 & 0.67 & 0.56 & 0.86 \\
 &  &  &  & 0.750000 & 0.80 & 0.81 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.20 & 0.22 & 0.80 \\
 &  &  &  & 0.500000 & 0.50 & 0.44 & 1.00 \\
 &  &  &  & 0.750000 & 0.75 & 0.78 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.25 & 0.22 & 0.86 \\
 &  &  &  & 0.500000 & 0.50 & 0.45 & 1.00 \\
 &  &  &  & 0.750000 & 0.78 & 0.78 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.25 \\
 &  &  &  & 0.750000 & 0.57 & 0.22 & 0.50 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.00 & 0.00 & 0.24 \\
 &  &  &  & 0.500000 & 0.00 & 0.18 & 0.50 \\
 &  &  &  & 0.750000 & 0.81 & 0.47 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & -0.09 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.27 \\
 &  &  &  & 0.750000 & 0.46 & 0.35 & 0.57 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.10 & 0.50 \\
 &  &  &  & 0.750000 & 0.00 & 0.33 & 0.75 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & -0.07 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.25 \\
 &  &  &  & 0.750000 & 0.10 & 0.21 & 0.50 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{30}{*}{7} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.50 & 0.19 & 0.67 \\
 &  &  &  & 0.500000 & 0.67 & 0.31 & 0.80 \\
 &  &  &  & 0.750000 & 0.80 & 0.54 & 0.91 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.46 & 0.31 & 0.70 \\
 &  &  &  & 0.500000 & 0.82 & 0.50 & 0.95 \\
 &  &  &  & 0.750000 & 1.00 & 0.64 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.50 & 0.25 & 0.80 \\
 &  &  &  & 0.500000 & 0.63 & 0.43 & 0.91 \\
 &  &  &  & 0.750000 & 0.76 & 0.77 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.25 & 0.23 & 0.76 \\
 &  &  &  & 0.500000 & 0.44 & 0.33 & 0.90 \\
 &  &  &  & 0.750000 & 0.73 & 0.57 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.50 & 0.31 & 0.80 \\
 &  &  &  & 0.500000 & 0.71 & 0.62 & 1.00 \\
 &  &  &  & 0.750000 & 0.91 & 0.92 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.31 & 0.18 \\
 &  &  &  & 0.750000 & 0.92 & 0.43 & 0.60 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.00 & 0.02 & 0.25 \\
 &  &  &  & 0.500000 & 0.00 & 0.23 & 0.45 \\
 &  &  &  & 0.750000 & 1.00 & 0.68 & 0.96 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.00 & 0.05 \\
 &  &  &  & 0.500000 & 0.00 & 0.08 & 0.38 \\
 &  &  &  & 0.750000 & 0.64 & 0.44 & 0.90 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.00 & 0.00 & 0.33 \\
 &  &  &  & 0.750000 & 0.00 & 0.14 & 0.55 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.08 & 0.00 \\
 &  &  &  & 0.500000 & 0.17 & 0.08 & 0.20 \\
 &  &  &  & 0.750000 & 0.77 & 0.27 & 0.40 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{2} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.60 & 0.61 & 0.85 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.56 & 0.58 & 0.88 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.49 & 0.56 & 0.85 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.51 & 0.59 & 0.88 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.46 & 0.54 & 0.87 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.24 & 0.20 & 0.21 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.14 & 0.16 & 0.26 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.09 & 0.12 & 0.22 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.06 & 0.14 & 0.31 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.14 & 0.18 & 0.27 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{3} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.68 & 0.60 & 0.91 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.62 & 0.57 & 0.91 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.59 & 0.49 & 0.84 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.49 & 0.53 & 0.88 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.51 & 0.52 & 0.86 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.25 & 0.19 & 0.27 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.20 & 0.21 & 0.39 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.11 & 0.07 & 0.21 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.05 & 0.14 & 0.38 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.15 & 0.13 & 0.24 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{5} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.64 & 0.52 & 0.82 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.61 & 0.53 & 0.86 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.60 & 0.54 & 0.86 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.47 & 0.49 & 0.88 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.52 & 0.50 & 0.87 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.24 & 0.13 & 0.30 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.30 & 0.28 & 0.52 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.22 & 0.17 & 0.36 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.06 & 0.16 & 0.46 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.15 & 0.11 & 0.28 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{7} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.67 & 0.38 & 0.81 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.71 & 0.53 & 0.86 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.61 & 0.49 & 0.84 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.47 & 0.41 & 0.84 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.66 & 0.59 & 0.87 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.41 & 0.25 & 0.35 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.43 & 0.36 & 0.54 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.26 & 0.27 & 0.46 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.05 & 0.09 & 0.35 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.33 & 0.21 & 0.27 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\bottomrule
\end{tabular}
\end{table}


==> generated/tables/compare_model_Yago.tex <==
\begin{table}
\caption{Comparison of models for Yago}
\label{tab:compare_model_Yago}
\begin{tabular}{lllllrrr}
\toprule
 &  &  &  &  & $F_{1,node}$ & $GED_{s}$ & $F_{1,rel.}$  \\
$k$ & Stage & Prompt Type & Version \& Size & Percentile &  &  &  \\
\midrule
\multirow[t]{30}{*}{2} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.50 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.50 & 0.60 & 1.00 \\
 &  &  &  & 0.500000 & 1.00 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.27 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 0.50 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.50 & 0.40 & 1.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.50 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.750000 & 0.67 & 0.33 & 0.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.50 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 0.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.50 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.750000 & 0.50 & 0.33 & 0.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 0.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 0.00 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{30}{*}{3} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.38 & 0.33 & 0.67 \\
 &  &  &  & 0.500000 & 0.67 & 0.50 & 1.00 \\
 &  &  &  & 0.750000 & 0.80 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.47 & 0.52 & 0.70 \\
 &  &  &  & 0.500000 & 0.80 & 0.80 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.40 & 0.33 & 0.54 \\
 &  &  &  & 0.500000 & 0.67 & 0.46 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.33 & 0.40 & 0.67 \\
 &  &  &  & 0.500000 & 0.67 & 0.60 & 1.00 \\
 &  &  &  & 0.750000 & 0.80 & 0.80 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.40 & 0.20 & 0.50 \\
 &  &  &  & 0.500000 & 0.67 & 0.54 & 0.67 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.33 & 0.19 & 0.00 \\
 &  &  &  & 0.500000 & 0.40 & 0.29 & 0.00 \\
 &  &  &  & 0.750000 & 0.67 & 0.40 & 0.50 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.44 & 0.33 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.40 & 0.40 \\
 &  &  &  & 0.750000 & 1.00 & 0.78 & 0.67 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.40 & 0.17 & 0.00 \\
 &  &  &  & 0.500000 & 0.67 & 0.22 & 0.00 \\
 &  &  &  & 0.750000 & 0.75 & 0.40 & 0.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.33 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.67 & 0.40 & 0.00 \\
 &  &  &  & 0.750000 & 0.67 & 0.60 & 0.50 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.40 & 0.38 & 0.00 \\
 &  &  &  & 0.500000 & 0.67 & 0.40 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.60 & 0.50 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{30}{*}{5} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.55 & 0.22 & 0.40 \\
 &  &  &  & 0.500000 & 0.60 & 0.44 & 0.86 \\
 &  &  &  & 0.750000 & 0.80 & 0.70 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.67 & 0.33 & 0.75 \\
 &  &  &  & 0.500000 & 0.89 & 0.70 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.94 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.50 & 0.22 & 0.43 \\
 &  &  &  & 0.500000 & 0.74 & 0.44 & 0.80 \\
 &  &  &  & 0.750000 & 0.89 & 0.76 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.50 & 0.40 & 0.78 \\
 &  &  &  & 0.500000 & 0.74 & 0.58 & 1.00 \\
 &  &  &  & 0.750000 & 0.87 & 0.78 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.67 & 0.29 & 0.57 \\
 &  &  &  & 0.500000 & 0.80 & 0.58 & 0.86 \\
 &  &  &  & 0.750000 & 1.00 & 0.89 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.40 & 0.11 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.26 & 0.25 \\
 &  &  &  & 0.750000 & 0.67 & 0.44 & 0.50 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.60 & 0.25 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.44 & 0.44 \\
 &  &  &  & 0.750000 & 1.00 & 0.83 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.40 & 0.11 & 0.00 \\
 &  &  &  & 0.500000 & 0.69 & 0.30 & 0.00 \\
 &  &  &  & 0.750000 & 0.80 & 0.44 & 0.25 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.44 & 0.11 & 0.00 \\
 &  &  &  & 0.500000 & 0.70 & 0.33 & 0.25 \\
 &  &  &  & 0.750000 & 0.80 & 0.65 & 0.50 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.60 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.44 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 0.50 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{30}{*}{7} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.55 & 0.23 & 0.06 \\
 &  &  &  & 0.500000 & 0.67 & 0.38 & 0.80 \\
 &  &  &  & 0.750000 & 0.73 & 0.67 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.83 & 0.69 & 0.91 \\
 &  &  &  & 0.500000 & 0.92 & 0.85 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.62 & 0.08 & 0.00 \\
 &  &  &  & 0.500000 & 0.83 & 0.38 & 0.67 \\
 &  &  &  & 0.750000 & 0.92 & 0.76 & 0.91 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.57 & 0.57 & 0.91 \\
 &  &  &  & 0.500000 & 0.71 & 0.69 & 1.00 \\
 &  &  &  & 0.750000 & 0.83 & 0.85 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.52 & 0.51 & 0.81 \\
 &  &  &  & 0.500000 & 0.75 & 0.69 & 0.95 \\
 &  &  &  & 0.750000 & 0.90 & 0.92 & 1.00 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.46 & 0.23 & 0.04 \\
 &  &  &  & 0.500000 & 0.55 & 0.38 & 0.27 \\
 &  &  &  & 0.750000 & 0.67 & 0.60 & 0.67 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.77 & 0.40 & 0.17 \\
 &  &  &  & 0.500000 & 0.83 & 0.62 & 0.50 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.67 & 0.31 & 0.00 \\
 &  &  &  & 0.500000 & 0.77 & 0.46 & 0.00 \\
 &  &  &  & 0.750000 & 0.86 & 0.52 & 0.20 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.46 & 0.31 & 0.17 \\
 &  &  &  & 0.500000 & 0.67 & 0.46 & 0.33 \\
 &  &  &  & 0.750000 & 0.83 & 0.77 & 1.00 \\
\cline{4-8}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.63 & 0.25 & 0.17 \\
 &  &  &  & 0.500000 & 0.77 & 0.54 & 0.43 \\
 &  &  &  & 0.750000 & 0.89 & 0.92 & 1.00 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{2} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.58 & 0.62 & 0.82 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.75 & 0.73 & 0.90 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.48 & 0.50 & 0.70 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.62 & 0.68 & 0.90 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.62 & 0.60 & 0.80 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.54 & 0.34 & 0.04 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.61 & 0.39 & 0.11 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.50 & 0.30 & 0.00 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.50 & 0.34 & 0.14 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.52 & 0.33 & 0.09 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{3} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.62 & 0.51 & 0.75 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.73 & 0.67 & 0.86 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.65 & 0.53 & 0.74 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.57 & 0.60 & 0.84 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.65 & 0.53 & 0.71 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.49 & 0.30 & 0.22 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.72 & 0.53 & 0.39 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.61 & 0.31 & 0.09 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.53 & 0.41 & 0.34 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.69 & 0.49 & 0.28 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{5} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.65 & 0.46 & 0.73 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.79 & 0.63 & 0.83 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.68 & 0.47 & 0.70 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.68 & 0.59 & 0.85 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.77 & 0.61 & 0.79 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.53 & 0.29 & 0.28 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.73 & 0.50 & 0.50 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.63 & 0.29 & 0.15 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.64 & 0.38 & 0.32 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.75 & 0.45 & 0.29 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\multirow[t]{10}{*}{7} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.64 & 0.44 & 0.61 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.87 & 0.78 & 0.91 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.79 & 0.43 & 0.52 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.69 & 0.69 & 0.92 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.71 & 0.66 & 0.82 \\
\cline{2-8} \cline{3-8} \cline{4-8}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.55 & 0.41 & 0.37 \\
\cline{4-8}
 &  &  & Hermes 3 70B & mean & 0.85 & 0.67 & 0.59 \\
\cline{4-8}
 &  &  & Hermes 3 8B & mean & 0.76 & 0.40 & 0.10 \\
\cline{4-8}
 &  &  & Qwen2.5 Coder 32B & mean & 0.65 & 0.54 & 0.54 \\
\cline{4-8}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.72 & 0.58 & 0.52 \\
\cline{1-8} \cline{2-8} \cline{3-8} \cline{4-8}
\bottomrule
\end{tabular}
\end{table}


==> generated/tables/compare_model_merged.tex <==
\begin{table}
\caption{Comparison of models for DBpedia and UniProt}
\label{tab:compare_model_merged}
\begin{tabular}{lllllrrrrrrrrrrrr}
\toprule
 &  &  &  &  & DBpedia $F_{1,node}$ & DBpedia $GED_{s}$ & $F_{1,rel.}$  & UniProt $F_{1,node}$ & UniProt $GED_{s}$ & UniProt $F_{1,rel.}$  & BTO $F_{1,node}$ & BTO $GED_{s}$ & BTO $F_{1,rel.}$  & Yago $F_{1,node}$ & Yago $GED_{s}$ & Yago $F_{1,rel.}$  \\
$k$ & Stage & Prompt Type & Version \& Size & Percentile &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[t]{30}{*}{2} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.50 & 0.25 & 0.00 & 0.50 & 0.33 & 1.00 & 0.00 & 0.33 & 1.00 & 0.50 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.67 & 1.00 & 0.50 & 0.67 & 1.00 & 0.00 & 0.33 & 1.00 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.50 & 0.67 & 1.00 & 1.00 & 1.00 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.50 & 0.33 & 0.00 & 0.40 & 0.33 & 1.00 & 0.00 & 0.33 & 1.00 & 0.50 & 0.60 & 1.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.40 & 1.00 & 0.50 & 0.67 & 1.00 & 0.50 & 0.33 & 1.00 & 1.00 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 & 1.00 & 1.00 & 1.00 & 0.67 & 0.67 & 1.00 & 1.00 & 1.00 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.14 & 0.00 & 0.00 & 0.33 & 1.00 & 0.00 & 0.33 & 1.00 & 0.00 & 0.27 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.33 & 1.00 & 0.50 & 0.67 & 1.00 & 0.00 & 0.33 & 1.00 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 & 1.00 & 0.67 & 1.00 & 0.50 & 0.33 & 1.00 & 0.50 & 0.67 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.20 & 0.00 & 0.00 & 0.33 & 1.00 & 0.00 & 0.33 & 1.00 & 0.50 & 0.40 & 1.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.40 & 1.00 & 0.50 & 0.67 & 1.00 & 0.00 & 0.33 & 1.00 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 & 1.00 & 0.67 & 1.00 & 0.50 & 0.67 & 1.00 & 1.00 & 1.00 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.33 & 0.00 & 0.00 & 0.33 & 1.00 & 0.00 & 0.33 & 1.00 & 0.50 & 0.33 & 1.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.45 & 1.00 & 0.50 & 0.67 & 1.00 & 0.00 & 0.33 & 1.00 & 0.50 & 0.67 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 & 0.67 & 0.67 & 1.00 & 0.50 & 0.33 & 1.00 & 1.00 & 1.00 & 1.00 \\
\cline{2-17} \cline{3-17} \cline{4-17}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.50 & 0.33 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.50 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 & 0.50 & 0.33 & 0.00 & 1.00 & 0.67 & 0.00 & 0.67 & 0.33 & 0.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.40 & 0.20 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.50 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.40 & 0.67 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 & 0.00 & 0.33 & 0.67 & 0.50 & 0.33 & 1.00 & 1.00 & 0.67 & 0.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.50 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.33 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 0.67 & 0.00 & 0.22 & 0.00 & 0.00 & 0.00 & 0.00 & 0.50 & 0.33 & 0.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.33 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 & 0.00 & 0.33 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.67 & 0.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
 &  &  &  & 0.500000 & 0.50 & 0.20 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.50 & 0.33 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 0.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 0.00 & 1.00 & 0.67 & 0.00 \\
\cline{1-17} \cline{2-17} \cline{3-17} \cline{4-17}
\multirow[t]{30}{*}{3} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.67 & 0.29 & 0.50 & 0.40 & 0.40 & 1.00 & 0.40 & 0.40 & 0.67 & 0.38 & 0.33 & 0.67 \\
 &  &  &  & 0.500000 & 0.80 & 0.50 & 0.80 & 0.80 & 0.60 & 1.00 & 0.67 & 0.60 & 1.00 & 0.67 & 0.50 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 & 1.00 & 0.83 & 1.00 & 1.00 & 0.80 & 1.00 & 0.80 & 0.80 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.67 & 0.22 & 0.50 & 0.33 & 0.33 & 1.00 & 0.50 & 0.33 & 0.67 & 0.47 & 0.52 & 0.70 \\
 &  &  &  & 0.500000 & 0.80 & 0.56 & 0.80 & 0.67 & 0.57 & 1.00 & 0.67 & 0.63 & 1.00 & 0.80 & 0.80 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.40 & 0.20 & 0.50 & 0.33 & 0.29 & 0.67 & 0.40 & 0.40 & 0.50 & 0.40 & 0.33 & 0.54 \\
 &  &  &  & 0.500000 & 0.80 & 0.50 & 0.67 & 0.67 & 0.40 & 1.00 & 0.67 & 0.60 & 1.00 & 0.67 & 0.46 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 & 1.00 & 0.80 & 1.00 & 1.00 & 0.80 & 1.00 & 1.00 & 0.80 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.40 & 0.33 & 0.50 & 0.00 & 0.29 & 0.83 & 0.40 & 0.40 & 1.00 & 0.33 & 0.40 & 0.67 \\
 &  &  &  & 0.500000 & 0.67 & 0.57 & 0.80 & 0.40 & 0.43 & 1.00 & 0.67 & 0.60 & 1.00 & 0.67 & 0.60 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 & 0.80 & 0.80 & 1.00 & 0.80 & 0.80 & 1.00 & 0.80 & 0.80 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.40 & 0.29 & 0.50 & 0.27 & 0.20 & 0.67 & 0.00 & 0.22 & 0.67 & 0.40 & 0.20 & 0.50 \\
 &  &  &  & 0.500000 & 0.67 & 0.50 & 1.00 & 0.50 & 0.40 & 1.00 & 0.33 & 0.40 & 1.00 & 0.67 & 0.54 & 0.67 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 & 1.00 & 0.80 & 1.00 & 0.73 & 0.60 & 1.00 & 1.00 & 0.80 & 1.00 \\
\cline{2-17} \cline{3-17} \cline{4-17}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.67 & 0.20 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.33 & 0.19 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.40 & 0.33 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.40 & 0.29 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.60 & 1.00 & 0.55 & 0.40 & 0.50 & 0.40 & 0.57 & 0.50 & 0.67 & 0.40 & 0.50 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.67 & 0.29 & 0.21 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.44 & 0.33 & 0.00 \\
 &  &  &  & 0.500000 & 0.93 & 0.57 & 0.67 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.80 & 0.40 & 0.40 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 & 0.00 & 0.40 & 1.00 & 0.00 & 0.38 & 0.50 & 1.00 & 0.78 & 0.67 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.50 & 0.20 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.40 & 0.17 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.40 & 0.40 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.67 & 0.22 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.60 & 0.80 & 0.00 & 0.20 & 0.50 & 0.00 & 0.14 & 0.00 & 0.75 & 0.40 & 0.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.40 & 0.20 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.33 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.67 & 0.40 & 0.50 & 0.00 & 0.00 & 0.40 & 0.00 & 0.00 & 0.00 & 0.67 & 0.40 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.80 & 1.00 & 0.00 & 0.40 & 0.73 & 0.00 & 0.21 & 0.75 & 0.67 & 0.60 & 0.50 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.33 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.40 & 0.38 & 0.00 \\
 &  &  &  & 0.500000 & 0.67 & 0.29 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.67 & 0.40 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.60 & 0.40 & 0.00 & 0.20 & 0.50 & 0.00 & 0.21 & 0.50 & 1.00 & 0.60 & 0.50 \\
\cline{1-17} \cline{2-17} \cline{3-17} \cline{4-17}
\multirow[t]{30}{*}{5} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.67 & 0.25 & 0.60 & 0.50 & 0.33 & 0.67 & 0.50 & 0.17 & 0.40 & 0.55 & 0.22 & 0.40 \\
 &  &  &  & 0.500000 & 0.80 & 0.44 & 0.80 & 0.67 & 0.44 & 0.86 & 0.60 & 0.33 & 0.67 & 0.60 & 0.44 & 0.86 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 & 0.80 & 0.78 & 1.00 & 0.80 & 0.83 & 1.00 & 0.80 & 0.70 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.67 & 0.22 & 0.60 & 0.43 & 0.33 & 0.75 & 0.44 & 0.33 & 0.67 & 0.67 & 0.33 & 0.75 \\
 &  &  &  & 0.500000 & 0.89 & 0.45 & 0.80 & 0.60 & 0.48 & 0.86 & 0.67 & 0.44 & 1.00 & 0.89 & 0.70 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.70 & 1.00 & 1.00 & 0.78 & 1.00 & 1.00 & 0.86 & 1.00 & 1.00 & 0.94 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.60 & 0.26 & 0.57 & 0.38 & 0.32 & 0.73 & 0.59 & 0.33 & 0.86 & 0.50 & 0.22 & 0.43 \\
 &  &  &  & 0.500000 & 0.80 & 0.44 & 0.75 & 0.67 & 0.56 & 0.86 & 0.75 & 0.51 & 0.86 & 0.74 & 0.44 & 0.80 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 & 0.80 & 0.81 & 1.00 & 0.82 & 0.72 & 1.00 & 0.89 & 0.76 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.50 & 0.25 & 0.57 & 0.20 & 0.22 & 0.80 & 0.52 & 0.31 & 0.75 & 0.50 & 0.40 & 0.78 \\
 &  &  &  & 0.500000 & 0.80 & 0.45 & 0.75 & 0.50 & 0.44 & 1.00 & 0.67 & 0.53 & 0.86 & 0.74 & 0.58 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.70 & 1.00 & 0.75 & 0.78 & 1.00 & 0.77 & 0.67 & 1.00 & 0.87 & 0.78 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.44 & 0.22 & 0.67 & 0.25 & 0.22 & 0.86 & 0.25 & 0.22 & 0.75 & 0.67 & 0.29 & 0.57 \\
 &  &  &  & 0.500000 & 0.75 & 0.45 & 0.75 & 0.50 & 0.45 & 1.00 & 0.40 & 0.40 & 0.86 & 0.80 & 0.58 & 0.86 \\
 &  &  &  & 0.750000 & 1.00 & 0.78 & 1.00 & 0.78 & 0.78 & 1.00 & 0.57 & 0.56 & 1.00 & 1.00 & 0.89 & 1.00 \\
\cline{2-17} \cline{3-17} \cline{4-17}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.60 & 0.13 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.40 & 0.11 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.30 & 0.29 & 0.00 & 0.00 & 0.25 & 0.00 & 0.00 & 0.00 & 0.50 & 0.26 & 0.25 \\
 &  &  &  & 0.750000 & 1.00 & 0.55 & 0.80 & 0.57 & 0.22 & 0.50 & 0.43 & 0.58 & 0.75 & 0.67 & 0.44 & 0.50 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.67 & 0.22 & 0.25 & 0.00 & 0.00 & 0.24 & 0.00 & 0.00 & 0.00 & 0.60 & 0.25 & 0.00 \\
 &  &  &  & 0.500000 & 0.89 & 0.45 & 0.67 & 0.00 & 0.18 & 0.50 & 0.00 & 0.00 & 0.00 & 0.80 & 0.44 & 0.44 \\
 &  &  &  & 0.750000 & 1.00 & 0.70 & 1.00 & 0.81 & 0.47 & 1.00 & 0.50 & 0.44 & 1.00 & 1.00 & 0.83 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.59 & 0.11 & 0.00 & 0.00 & -0.09 & 0.00 & 0.00 & 0.00 & 0.00 & 0.40 & 0.11 & 0.00 \\
 &  &  &  & 0.500000 & 0.80 & 0.33 & 0.25 & 0.00 & 0.00 & 0.27 & 0.00 & 0.00 & 0.00 & 0.69 & 0.30 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.56 & 0.75 & 0.46 & 0.35 & 0.57 & 0.00 & 0.38 & 0.89 & 0.80 & 0.44 & 0.25 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.44 & 0.11 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -0.10 & 0.00 & 0.44 & 0.11 & 0.00 \\
 &  &  &  & 0.500000 & 0.75 & 0.33 & 0.25 & 0.00 & 0.10 & 0.50 & 0.00 & 0.00 & 0.00 & 0.70 & 0.33 & 0.25 \\
 &  &  &  & 0.750000 & 1.00 & 0.60 & 1.00 & 0.00 & 0.33 & 0.75 & 0.00 & 0.44 & 1.00 & 0.80 & 0.65 & 0.50 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.29 & 0.10 & 0.00 & 0.00 & -0.07 & 0.00 & 0.00 & -0.10 & 0.00 & 0.60 & 0.20 & 0.00 \\
 &  &  &  & 0.500000 & 0.67 & 0.27 & 0.00 & 0.00 & 0.00 & 0.25 & 0.00 & 0.00 & 0.00 & 0.80 & 0.44 & 0.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.56 & 0.75 & 0.10 & 0.21 & 0.50 & 0.00 & 0.44 & 1.00 & 1.00 & 0.67 & 0.50 \\
\cline{1-17} \cline{2-17} \cline{3-17} \cline{4-17}
\multirow[t]{30}{*}{7} & \multirow[t]{15}{*}{aligned} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.55 & 0.17 & 0.55 & 0.50 & 0.19 & 0.67 & 0.67 & 0.56 & 0.63 & 0.55 & 0.23 & 0.06 \\
 &  &  &  & 0.500000 & 0.73 & 0.31 & 0.80 & 0.67 & 0.31 & 0.80 & 0.72 & 0.58 & 0.66 & 0.67 & 0.38 & 0.80 \\
 &  &  &  & 0.750000 & 0.91 & 0.54 & 0.92 & 0.80 & 0.54 & 0.91 & 0.78 & 0.60 & 0.70 & 0.73 & 0.67 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.61 & 0.20 & 0.60 & 0.46 & 0.31 & 0.70 & 0.33 & 0.25 & 0.67 & 0.83 & 0.69 & 0.91 \\
 &  &  &  & 0.500000 & 0.86 & 0.43 & 0.83 & 0.82 & 0.50 & 0.95 & 0.67 & 0.33 & 0.80 & 0.92 & 0.85 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.67 & 1.00 & 1.00 & 0.64 & 1.00 & 0.86 & 0.57 & 1.00 & 1.00 & 1.00 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.60 & 0.21 & 0.55 & 0.50 & 0.25 & 0.80 & 0.50 & 0.16 & 0.58 & 0.62 & 0.08 & 0.00 \\
 &  &  &  & 0.500000 & 0.83 & 0.38 & 0.80 & 0.63 & 0.43 & 0.91 & 0.64 & 0.31 & 0.72 & 0.83 & 0.38 & 0.67 \\
 &  &  &  & 0.750000 & 0.92 & 0.60 & 0.91 & 0.76 & 0.77 & 1.00 & 0.78 & 0.47 & 0.86 & 0.92 & 0.76 & 0.91 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.55 & 0.24 & 0.62 & 0.25 & 0.23 & 0.76 & 0.62 & 0.77 & 1.00 & 0.57 & 0.57 & 0.91 \\
 &  &  &  & 0.500000 & 0.83 & 0.38 & 0.83 & 0.44 & 0.33 & 0.90 & 0.62 & 0.77 & 1.00 & 0.71 & 0.69 & 1.00 \\
 &  &  &  & 0.750000 & 1.00 & 0.64 & 1.00 & 0.73 & 0.57 & 1.00 & 0.62 & 0.77 & 1.00 & 0.83 & 0.85 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.44 & 0.25 & 0.60 & 0.50 & 0.31 & 0.80 & 0.29 & 0.48 & 0.85 & 0.52 & 0.51 & 0.81 \\
 &  &  &  & 0.500000 & 0.75 & 0.44 & 0.83 & 0.71 & 0.62 & 1.00 & 0.39 & 0.58 & 0.90 & 0.75 & 0.69 & 0.95 \\
 &  &  &  & 0.750000 & 1.00 & 0.69 & 1.00 & 0.91 & 0.92 & 1.00 & 0.48 & 0.67 & 0.95 & 0.90 & 0.92 & 1.00 \\
\cline{2-17} \cline{3-17} \cline{4-17}
 & \multirow[t]{15}{*}{raw} & \multirow[t]{15}{*}{one shot} & \multirow[t]{3}{*}{Hermes 3 3B} & 0.250000 & 0.60 & 0.08 & 0.15 & 0.00 & 0.00 & 0.00 & 0.21 & 0.19 & 0.17 & 0.46 & 0.23 & 0.04 \\
 &  &  &  & 0.500000 & 0.77 & 0.27 & 0.33 & 0.00 & 0.31 & 0.18 & 0.43 & 0.38 & 0.33 & 0.55 & 0.38 & 0.27 \\
 &  &  &  & 0.750000 & 0.86 & 0.46 & 0.83 & 0.92 & 0.43 & 0.60 & 0.64 & 0.58 & 0.50 & 0.67 & 0.60 & 0.67 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 70B} & 0.250000 & 0.71 & 0.22 & 0.20 & 0.00 & 0.02 & 0.25 & 0.00 & 0.00 & 0.00 & 0.77 & 0.40 & 0.17 \\
 &  &  &  & 0.500000 & 0.86 & 0.38 & 0.62 & 0.00 & 0.23 & 0.45 & 0.00 & 0.00 & 0.00 & 0.83 & 0.62 & 0.50 \\
 &  &  &  & 0.750000 & 1.00 & 0.62 & 1.00 & 1.00 & 0.68 & 0.96 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Hermes 3 8B} & 0.250000 & 0.67 & 0.14 & 0.00 & 0.00 & 0.00 & 0.05 & 0.00 & 0.10 & 0.23 & 0.67 & 0.31 & 0.00 \\
 &  &  &  & 0.500000 & 0.83 & 0.31 & 0.33 & 0.00 & 0.08 & 0.38 & 0.00 & 0.20 & 0.46 & 0.77 & 0.46 & 0.00 \\
 &  &  &  & 0.750000 & 0.92 & 0.50 & 0.83 & 0.64 & 0.44 & 0.90 & 0.00 & 0.30 & 0.69 & 0.86 & 0.52 & 0.20 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Coder 32B} & 0.250000 & 0.55 & 0.13 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.46 & 1.00 & 0.46 & 0.31 & 0.17 \\
 &  &  &  & 0.500000 & 0.83 & 0.31 & 0.40 & 0.00 & 0.00 & 0.33 & 0.00 & 0.46 & 1.00 & 0.67 & 0.46 & 0.33 \\
 &  &  &  & 0.750000 & 1.00 & 0.62 & 1.00 & 0.00 & 0.14 & 0.55 & 0.00 & 0.46 & 1.00 & 0.83 & 0.77 & 1.00 \\
\cline{4-17}
 &  &  & \multirow[t]{3}{*}{Qwen2.5 Instruct 32B} & 0.250000 & 0.36 & 0.08 & 0.00 & 0.00 & 0.08 & 0.00 & 0.00 & 0.12 & 0.25 & 0.63 & 0.25 & 0.17 \\
 &  &  &  & 0.500000 & 0.62 & 0.27 & 0.00 & 0.17 & 0.08 & 0.20 & 0.00 & 0.23 & 0.50 & 0.77 & 0.54 & 0.43 \\
 &  &  &  & 0.750000 & 0.93 & 0.54 & 0.92 & 0.77 & 0.27 & 0.40 & 0.00 & 0.35 & 0.75 & 0.89 & 0.92 & 1.00 \\
\cline{1-17} \cline{2-17} \cline{3-17} \cline{4-17}
\multirow[t]{10}{*}{2} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.67 & 0.57 & 0.62 & 0.60 & 0.61 & 0.85 & 0.28 & 0.43 & 0.80 & 0.58 & 0.62 & 0.82 \\
\cline{4-17}
 &  &  & Hermes 3 70B & mean & 0.64 & 0.53 & 0.67 & 0.56 & 0.58 & 0.88 & 0.41 & 0.49 & 0.83 & 0.75 & 0.73 & 0.90 \\
\cline{4-17}
 &  &  & Hermes 3 8B & mean & 0.48 & 0.47 & 0.62 & 0.49 & 0.56 & 0.85 & 0.18 & 0.35 & 0.78 & 0.48 & 0.50 & 0.70 \\
\cline{4-17}
 &  &  & Qwen2.5 Coder 32B & mean & 0.49 & 0.50 & 0.66 & 0.51 & 0.59 & 0.88 & 0.33 & 0.46 & 0.82 & 0.62 & 0.68 & 0.90 \\
\cline{4-17}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.51 & 0.51 & 0.64 & 0.46 & 0.54 & 0.87 & 0.19 & 0.39 & 0.82 & 0.62 & 0.60 & 0.80 \\
\cline{2-17} \cline{3-17} \cline{4-17}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.68 & 0.51 & 0.41 & 0.24 & 0.20 & 0.21 & 0.35 & 0.27 & 0.18 & 0.54 & 0.34 & 0.04 \\
\cline{4-17}
 &  &  & Hermes 3 70B & mean & 0.65 & 0.49 & 0.47 & 0.14 & 0.16 & 0.26 & 0.21 & 0.23 & 0.33 & 0.61 & 0.39 & 0.11 \\
\cline{4-17}
 &  &  & Hermes 3 8B & mean & 0.49 & 0.38 & 0.32 & 0.09 & 0.12 & 0.22 & 0.01 & 0.06 & 0.16 & 0.50 & 0.30 & 0.00 \\
\cline{4-17}
 &  &  & Qwen2.5 Coder 32B & mean & 0.44 & 0.39 & 0.39 & 0.06 & 0.14 & 0.31 & 0.01 & 0.07 & 0.19 & 0.50 & 0.34 & 0.14 \\
\cline{4-17}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.45 & 0.31 & 0.14 & 0.14 & 0.18 & 0.27 & 0.05 & 0.10 & 0.21 & 0.52 & 0.33 & 0.09 \\
\cline{1-17} \cline{2-17} \cline{3-17} \cline{4-17}
\multirow[t]{10}{*}{3} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.75 & 0.52 & 0.68 & 0.68 & 0.60 & 0.91 & 0.65 & 0.59 & 0.73 & 0.62 & 0.51 & 0.75 \\
\cline{4-17}
 &  &  & Hermes 3 70B & mean & 0.75 & 0.53 & 0.69 & 0.62 & 0.57 & 0.91 & 0.65 & 0.61 & 0.77 & 0.73 & 0.67 & 0.86 \\
\cline{4-17}
 &  &  & Hermes 3 8B & mean & 0.71 & 0.51 & 0.65 & 0.59 & 0.49 & 0.84 & 0.66 & 0.59 & 0.73 & 0.65 & 0.53 & 0.74 \\
\cline{4-17}
 &  &  & Qwen2.5 Coder 32B & mean & 0.66 & 0.54 & 0.71 & 0.49 & 0.53 & 0.88 & 0.59 & 0.63 & 0.91 & 0.57 & 0.60 & 0.84 \\
\cline{4-17}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.64 & 0.53 & 0.71 & 0.51 & 0.52 & 0.86 & 0.37 & 0.46 & 0.83 & 0.65 & 0.53 & 0.71 \\
\cline{2-17} \cline{3-17} \cline{4-17}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.75 & 0.43 & 0.40 & 0.25 & 0.19 & 0.27 & 0.24 & 0.20 & 0.24 & 0.49 & 0.30 & 0.22 \\
\cline{4-17}
 &  &  & Hermes 3 70B & mean & 0.77 & 0.55 & 0.60 & 0.20 & 0.21 & 0.39 & 0.22 & 0.22 & 0.25 & 0.72 & 0.53 & 0.39 \\
\cline{4-17}
 &  &  & Hermes 3 8B & mean & 0.71 & 0.42 & 0.38 & 0.11 & 0.07 & 0.21 & 0.05 & 0.07 & 0.20 & 0.61 & 0.31 & 0.09 \\
\cline{4-17}
 &  &  & Qwen2.5 Coder 32B & mean & 0.63 & 0.43 & 0.44 & 0.05 & 0.14 & 0.38 & 0.00 & 0.09 & 0.27 & 0.53 & 0.41 & 0.34 \\
\cline{4-17}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.58 & 0.34 & 0.21 & 0.15 & 0.13 & 0.24 & 0.07 & 0.14 & 0.27 & 0.69 & 0.49 & 0.28 \\
\cline{1-17} \cline{2-17} \cline{3-17} \cline{4-17}
\multirow[t]{10}{*}{5} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.75 & 0.45 & 0.74 & 0.64 & 0.52 & 0.82 & 0.60 & 0.46 & 0.68 & 0.65 & 0.46 & 0.73 \\
\cline{4-17}
 &  &  & Hermes 3 70B & mean & 0.80 & 0.48 & 0.75 & 0.61 & 0.53 & 0.86 & 0.63 & 0.55 & 0.80 & 0.79 & 0.63 & 0.83 \\
\cline{4-17}
 &  &  & Hermes 3 8B & mean & 0.73 & 0.46 & 0.73 & 0.60 & 0.54 & 0.86 & 0.72 & 0.55 & 0.84 & 0.68 & 0.47 & 0.70 \\
\cline{4-17}
 &  &  & Qwen2.5 Coder 32B & mean & 0.70 & 0.48 & 0.77 & 0.47 & 0.49 & 0.88 & 0.63 & 0.49 & 0.81 & 0.68 & 0.59 & 0.85 \\
\cline{4-17}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.66 & 0.49 & 0.76 & 0.52 & 0.50 & 0.87 & 0.41 & 0.43 & 0.83 & 0.77 & 0.61 & 0.79 \\
\cline{2-17} \cline{3-17} \cline{4-17}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.76 & 0.35 & 0.42 & 0.24 & 0.13 & 0.30 & 0.23 & 0.23 & 0.32 & 0.53 & 0.29 & 0.28 \\
\cline{4-17}
 &  &  & Hermes 3 70B & mean & 0.80 & 0.48 & 0.60 & 0.30 & 0.28 & 0.52 & 0.26 & 0.27 & 0.31 & 0.73 & 0.50 & 0.50 \\
\cline{4-17}
 &  &  & Hermes 3 8B & mean & 0.71 & 0.35 & 0.40 & 0.22 & 0.17 & 0.36 & 0.07 & 0.18 & 0.38 & 0.63 & 0.29 & 0.15 \\
\cline{4-17}
 &  &  & Qwen2.5 Coder 32B & mean & 0.69 & 0.38 & 0.47 & 0.06 & 0.16 & 0.46 & 0.00 & 0.11 & 0.35 & 0.64 & 0.38 & 0.32 \\
\cline{4-17}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.61 & 0.32 & 0.30 & 0.15 & 0.11 & 0.28 & 0.01 & 0.12 & 0.34 & 0.75 & 0.45 & 0.29 \\
\cline{1-17} \cline{2-17} \cline{3-17} \cline{4-17}
\multirow[t]{10}{*}{7} & \multirow[t]{5}{*}{aligned} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.71 & 0.36 & 0.71 & 0.67 & 0.38 & 0.81 & 0.72 & 0.58 & 0.66 & 0.64 & 0.44 & 0.61 \\
\cline{4-17}
 &  &  & Hermes 3 70B & mean & 0.78 & 0.42 & 0.74 & 0.71 & 0.53 & 0.86 & 0.57 & 0.40 & 0.73 & 0.87 & 0.78 & 0.91 \\
\cline{4-17}
 &  &  & Hermes 3 8B & mean & 0.74 & 0.41 & 0.71 & 0.61 & 0.49 & 0.84 & 0.64 & 0.31 & 0.72 & 0.79 & 0.43 & 0.52 \\
\cline{4-17}
 &  &  & Qwen2.5 Coder 32B & mean & 0.75 & 0.44 & 0.77 & 0.47 & 0.41 & 0.84 & 0.62 & 0.77 & 1.00 & 0.69 & 0.69 & 0.92 \\
\cline{4-17}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.67 & 0.46 & 0.76 & 0.66 & 0.59 & 0.87 & 0.39 & 0.58 & 0.90 & 0.71 & 0.66 & 0.82 \\
\cline{2-17} \cline{3-17} \cline{4-17}
 & \multirow[t]{5}{*}{raw} & \multirow[t]{5}{*}{one shot} & Hermes 3 3B & mean & 0.72 & 0.30 & 0.46 & 0.41 & 0.25 & 0.35 & 0.43 & 0.38 & 0.33 & 0.55 & 0.41 & 0.37 \\
\cline{4-17}
 &  &  & Hermes 3 70B & mean & 0.80 & 0.42 & 0.60 & 0.43 & 0.36 & 0.54 & 0.09 & 0.02 & 0.04 & 0.85 & 0.67 & 0.59 \\
\cline{4-17}
 &  &  & Hermes 3 8B & mean & 0.76 & 0.33 & 0.43 & 0.26 & 0.27 & 0.46 & 0.00 & 0.20 & 0.46 & 0.76 & 0.40 & 0.10 \\
\cline{4-17}
 &  &  & Qwen2.5 Coder 32B & mean & 0.72 & 0.40 & 0.53 & 0.05 & 0.09 & 0.35 & 0.00 & 0.46 & 1.00 & 0.65 & 0.54 & 0.54 \\
\cline{4-17}
 &  &  & Qwen2.5 Instruct 32B & mean & 0.61 & 0.32 & 0.34 & 0.33 & 0.21 & 0.27 & 0.00 & 0.23 & 0.50 & 0.72 & 0.58 & 0.52 \\
\cline{1-17} \cline{2-17} \cline{3-17} \cline{4-17}
\bottomrule
\end{tabular}
\end{table}


==> generated/tables/task_results.tex <==
\begin{table}
\caption{Task results for the OnSET user study on DBpedia with $n=11$.}
\label{tab:task_results}
\begin{tabular}{lrl}
\toprule
Task & Success Rate & Time (mm:ss) \\
\midrule
Task 0 & 0.73 & 03:46 \\
Task 1 & 0.91 & 01:12 \\
Task 2 & 0.73 & 04:49 \\
Task 3 & 1.00 & 02:05 \\
\bottomrule
\end{tabular}
\end{table}

